Nearly Optimal Algorithms for Level Set Estimation

The level set estimation problem seeks to find all points in a domain ${\cal X}$ where the value of an unknown function $f:{\cal X}\rightarrow \mathbb{R}$ exceeds a threshold $\alpha$. The estimation is based on noisy function evaluations that may be acquired at sequentially and adaptively chosen locations in ${\cal X}$. The threshold value $\alpha$ can either be \emph{explicit} and provided a priori, or \emph{implicit} and defined relative to the optimal function value, i.e. $\alpha = (1-\epsilon)f(x_\ast)$ for a given $\epsilon > 0$ where $f(x_\ast)$ is the maximal function value and is unknown. In this work we provide a new approach to the level set estimation problem by relating it to recent adaptive experimental design methods for linear bandits in the Reproducing Kernel Hilbert Space (RKHS) setting. We assume that $f$ can be approximated by a function in the RKHS up to an unknown misspecification and provide novel algorithms for both the implicit and explicit cases in this setting with strong theoretical guarantees. Moreover, in the linear (kernel) setting, we show that our bounds are nearly optimal, namely, our upper bounds match existing lower bounds for threshold linear bandits. To our knowledge this work provides the first instance-dependent, non-asymptotic upper bounds on sample complexity of level-set estimation that match information theoretic lower bounds.

==> fixed_budget.tex <==
\section{Fixed Budget Implict Level Set Estimation}

Finally, one may wish to identify the level set of a function they know very little about or may otherwise be challenging to model and removing structural assumptions and modelling the $\bx$'s as independent may be more reasonable. In this setting, level set estimation is reduces to standard multiarmed bandits. The explicit case is equivalent to the problem of thresholding bandits and optimal algorithms exist in the fixed confidence and fixed budget regime such as \citep{locatelli2016optimal, jamieson2018bandit}. In the implicit setting, \citep{mason2020finding} develop several optimal algorithms for fixed confidence. We provide a fixed budget algorithm for this setting to complement previous approaches. For consistency with the bandit literature, we take $\mu_i = f(\bx_i)$ to denote the mean of $\bx_i$ and without loss of generality, we assume that $\mu_1 \geq \cdots \geq \mu_n$ for $n = |\X|$. Throughout, we take $\hat{\mu}_i$ to denote the empirical mean of an arm $i$. 
The algorithm is given a budget of $T$ samples and wishes to identify the set of all $i$ such that $\mu_i \geq (1-\epsilon)\mu_1$ with as large of probability as possible. We refer to our algorithm as \texttt{LATTE}: \textbf{L}earn \textbf{A} \textbf{T}hreshold \textbf{T}hen \textbf{E}liminate\footnote{Latte is `milk' in Italian}. \texttt{LATTE} proceeds in three phases dividing the budget into equal parts. In the first phase, it identifies a nearly optimal arm $\hat{i}$. Note that it does not necessarily identify the optimal arm. Instead, we provide a new guarantee for fixed-budget $\epsilon$-good arm identification in multiarmed bandits. To do so, the algorithm divides the budget of $T/3$ samples for that phase into rounds of sampling and filters on gaps. The algorithm keeps track of a set of active arms $\B$. 
In round $k$, the algorithm samples each active arm \begin{align*}
    N_k = \dfrac{\psi\log(T\tDelta_m/3)}{2^{-k+1}}
\end{align*}
times
for a normalizing constant $\psi$ and then removes any arm satisfying
\begin{align*}
    \wmu_{i}(k) +  C_k(\tDelta_k, T) < \max_{j\in\B_k} \wmu_{j}(k) -  C_k(\tDelta_k, T)
\end{align*} 
for a confidence width
\begin{align*}
    C_m(\tDelta_m, T) = \sqrt{\dfrac{\psi\log(T(2^{-k}/3)}{2N_k}}.
\end{align*}
The phase terminates when the budget of $T/3$ samples exhausted and returns the active arm with the highest empirical mean $\hat{i}$. We make the assumption that the budget $T$ satisfies $\omega = \min_i |\mu_i - (1-\epsilon)\mu_1| \geq \sqrt{3e/T}$. In particular, if this constraint is not satisfied, any algorithm makes an error with constant probability in declaring whether the closest mean $\mu_i$ to the threshold $(1-\epsilon)\mu_i$ is or is not good. Hence, the assumption is mild.


In the next phase, the algorithm samples  $\hat{i}$ repeatedly repeatedly to learn a precise estimate of $(1-\epsilon)\mu_{\hat{i}}$. In the final phase, the algorithm uses $(1-\epsilon)\hat{\mu}_{\hat{i}}$ as an empirical estimate of the threshold $(1-\epsilon)\mu_1$ and follows the \texttt{APT} sampling policy of \citep{locatelli2016optimal} to separate arms from a fixed threshold. Finally, \texttt{LATTE} returns the arms declared to exceed the threshold. Psuedocode is given in Algorithm~\ref{alg:latte}. 

\begin{algorithm}[tbh]
\caption{\texttt{LATTE}: \textbf{L}earn \textbf{A} \textbf{T}hreshold \textbf{T}hen \textbf{E}liminate}
\label{alg:latte}
\begin{algorithmic}[1]
\State \textbf{Init:} Budget $T$, $\epsilon$, tolerance $\gamma$.
\State \textbf{Initialize:} Active set $\B_1 = \emptyset$.
\For{$m = 1, 2, \ldots, \frac{1}{2}\log_2\frac{T}{3e}$}\Comment{Gap Elim not-$w$ arms}
\State Pull each arm $i\in\B_m$ for $N_m$ times till $|\B_m| > 1$. If $|\B_m| = 1$ then sample arm $i\in\B_m$ until round $\frac{T}{3}$.
\State Remove arm $i$ from $\B_m$ using \eqref{eq:geapt-elim}
\State Set $\tDelta_m = \frac{\tDelta_m}{2}$, $m = m + 1$.
\EndFor
%\For{$t= \frac{T}{3} + 1, \frac{T}{3} + 2, \ldots, \frac{2T}{3}$} 
\State Let $i_w \in \B_M$. If $|\B_M| > 1$ then  choose $i_w \coloneqq \max_{j\in\B_M}\wmu_j$. \Comment{Sample $w$-good arm $\frac{T}{3}$ times}
\State Sample arm $i_w$ until $\frac{2T}{3}$ rounds.
%\EndFor
\For{$t= \frac{2T}{3} + 1, \frac{2T}{3} + 2, \ldots,T$}
\State Define threshold $\tau = \wmu_{i_w} - \epsilon$ \Comment{Set threshold $\tau$}
\State Define $\B_i(t) \coloneqq \sqrt{N_i(t)}\left(\left|\hat{\mu}_i(t) - \tau\right| + \gamma\right)$
\State Sample arm $i_{t} \argmin\limits_{i\in[K]} \B_i(t)$ \Comment{Run APT}
\EndFor
\State Output $\wS(T) \coloneqq \{i\in[K]: \wmu_i(t) \geq \tau\}$
\end{algorithmic} 
\end{algorithm} 

\subsection{Theoretical Guarantees}

\blake{To do: prove this result in the multiplicative case and come up with the combined theoretical guarantees for the three phases}

Then we define the problem complexity parameter $H^{\omega}_2$ as follows:
\begin{align}
    %H^{\omega}_2 = \max \left\{\min_i \{i\Delta^{-2}_{(i)}, w^{-2}\}\right\} 
    H^{\omega}_2 = \max i (\Delta^w_{(i)})^{-2} \label{eq:H2w}
\end{align}
where, $\Delta_{(i)}$ is $\Delta_i$ ordered in increasing order, and $\Delta^w_i = \max\{\Delta_i, w\}$.

\begin{theorem}
Let $\G_\epsilon \coloneqq \{i\in [K]: \mu_{i} \geq \mu_{i^*} - \epsilon\}$ is the set of all $\epsilon$-good arms. Define $Good \coloneqq \{\wS(T) = G_\epsilon\}$ as the event that \geAPT outputs all the $\epsilon$-good arms. Then the error probability that \geAPT outputs an arm that is not in $\G_\epsilon$ is bounded by
%, where $w \coloneqq \min_{i\in[K]}|\mu_i - (\mu_{i^*} - \epsilon)|$. Define $\xi_{final}$ as the probability of error that some not-$w$ arms are accepted as $w$-good arms at the end of the budget $T$. Then the probability of error when \Cref{alg:egAPT} is run on $[K]$ arms is given by
\begin{align*}
    \Pb(\neg Good) \leq O\left(KT\exp\left(-\frac{T }{ \log K H^{w}_2}\right)\right)
\end{align*}
where, $H^w_2$ is defined in \eqref{eq:H2w}.
\end{theorem}

